PI-Trans: Parallel-ConvMLP and Implicit-Transformation Based GAN for Cross-View Image Translation

For semantic-guided cross-view image translation, it is crucial to learn where to sample pixels from the source view image and where to reallocate them guided by the target view semantic map, especially when there is little overlap or drastic view difference between the source and target images. Hence, one not only needs to encode the long-range dependencies among pixels in both the source view image and target view semantic map but also needs to translate these learned dependencies. To this end, we propose a novel generative adversarial network, PI-Trans, which mainly consists of a novel Parallel-ConvMLP module and an Implicit Transformation module at multiple semantic levels. Extensive experimental results show that PI-Trans achieves the best qualitative and quantitative performance by a large margin compared to the state-of-the-art methods on two challenging datasets. The source code is available at https://github.com/Amazingren/PI-Trans.

==> sections/2relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\noindent\textbf{Cross-View Image Geo-localization.}
Image geo-localization has been tackled as an image matching task to tell the location of a query image by comparing it with geo-tagged database images~\cite{shi2019spatial,shi2020optimal}. Different from previous works that focus on the ground-to-ground image matching~\cite{arandjelovic2016netvlad,liu2019stochastic,sattler2019understanding}, recent works pay more attention to the cross-view setting where the query image is at ground level while the geo-tagged image gallery is captured by the satellite at the aerial view~\cite{zhu2021vigor,liu2019lending,hu2018cvm,cai2019ground}. Though the cross-view setting of geo-localization is promising at lots of computer vision tasks such as robot navigation, civil engineering design, as well as the way-finding in AR/VR applications, it's also challenging due to the vast differences in terms of both the appearances and the distinctive geometric configurations between the aerial-view and the ground-view images that from two drastic viewpoints. To this end,
Regmi \textit{et al.} proposes to use conditional GAN to generate an aerial image from its corresponding ground view panorama and use it for minimizing the domain gap between the drastic two views~\cite{regmi2019bridging}. Similarly, Toker \textit{et al.} also boosts the performance of geo-localization with the help of the generated ground-view panorama from its corresponding aerial-view image~\cite{toker2021coming}. Instead of using the global information like the entire panorama edge map used in~\cite{regmi2019bridging} or a polar transformation operation used in~\cite{toker2021coming} during the generation part in their methods, we use the cropped ground-view semantic map as the condition inputs, which is obvious isolated from the rest part and the information provided by the cropped semantic map is also limited. Consequently, the condition setting in our paper is more challenging for generating realistic cross-view images but more flexible because the target-view condition input is easier to acquire either from other modality or just elaborately designed by human.


\noindent\textbf{Cross-View Image Translation.}
Conditional GAN is a special generative model for generating new samples which have the desired data distributions with guidance from the conditioned information like class labels, attention maps, and so on~\cite{goodfellow2014generative}. In this paper, we adopt the random cropped ground-view semantic map as conditional information for cross-view image translation task.

Unlike most of the previous methods on cross-view image translation task that there exists a large degree of overlapping in both appearance or geometry structures~\cite{dosovitskiy2017learning,zhou2016view,he2019deliberation}. When the two views are dramatically different, this task certainly becomes very challenging since the severe discrepancy leads to lots of problems like geometry mismatch, scale uncertainty, and so on. Zhai \textit{et al.} firstly proposed a CNN-based framework to address this problem~\cite{zhai2017predicting}. Due to the target-view semantic map is easy to acquire from another modality. Regmi \textit{et al.} designed two GAN based structures X-Fork and X-Seq to further address this problem conditioned on the ground-view semantic map~\cite{regmi2018cross}. To further improve the performance, Tang \textit{et al.} proposed a two-stage framework which can generate better results based on its enlarged generation space~\cite{tang2019multi}. These two methods are all not good at modeling the long-range relation for the given input. Ren \textit{et al.} eased this problem with its cross MLP module progressively~\cite{ren2021cascaded}. Different from above approaches that completely rely on a deep learning architecture, Lu \textit{et al.} explicitly add the geometric configuration for cross-view image generation~\cite{lu2020geometry}, however, besides the semantic condition information, their method needs the depth information from both the aerial-view and the ground-view as supervision, which puts this task in a more expensive level. 

Most of these cross-view translation methods solely rely on the semantic condition guided generation as a ritual, and pay little attention to the information of the direct translation branch (shown in Fig.~\ref{fig:framework})  which actually could provides useful colour distribution to make the final generated ground view image sharper and more realistic. What's more, since in our setting, the condition information from the semantic map is just a small part of the entire panorama, it is even essential for the deep model to have a strong ability for modeling the long-range dependencies and the spatial information in both the given aerial images and the semantic maps under this global information limited situation. Hence, we aim to overcome these issues by the proposed PI-Trans under the support of the proposed parallel-ConvMLP and the implicit-transformation modules. 






